Another Shipment of Six Short-Period Giant Planets from TESS

We present the discovery and characterization of six short-period, transiting giant planets from NASA's Transiting Exoplanet Survey Satellite (TESS) -- TOI-1811 (TIC 376524552), TOI-2025 (TIC 394050135), TOI-2145 (TIC 88992642), TOI-2152 (TIC 395393265), TOI-2154 (TIC 428787891), & TOI-2497 (TIC 97568467). All six planets orbit bright host stars (8.9 <G< 11.8, 7.7 <K< 10.1). Using a combination of time-series photometric and spectroscopic follow-up observations from the TESS Follow-up Observing Program (TFOP) Working Group, we have determined that the planets are Jovian-sized (R$_{P}$ = 1.00-1.45 R$_{J}$), have masses ranging from 0.92 to 5.35 M$_{J}$, and orbit F, G, and K stars (4753 $<$ T$_{eff}$ $<$ 7360 K). We detect a significant orbital eccentricity for the three longest-period systems in our sample: TOI-2025 b (P = 8.872 days, $e$ = $0.220\pm0.053$), TOI-2145 b (P = 10.261 days, $e$ = $0.182^{+0.039}_{-0.049}$), and TOI-2497 b (P = 10.656 days, $e$ = $0.196^{+0.059}_{-0.053}$). TOI-2145 b and TOI-2497 b both orbit subgiant host stars (3.8 $<$ $\log$ g $<$4.0), but these planets show no sign of inflation despite very high levels of irradiation. The lack of inflation may be explained by the high mass of the planets; $5.35^{+0.32}_{-0.35}$ M$_{\rm J}$ (TOI-2145 b) and $5.21\pm0.52$ M$_{\rm J}$ (TOI-2497 b). These six new discoveries contribute to the larger community effort to use {\it TESS} to create a magnitude-complete, self-consistent sample of giant planets with well-determined parameters for future detailed studies.

==> Notes.tex <==
Comments: 
1) Take a look a Hughs aesthetic changes
2) TSM analysis 
3) P=4.72 days box is slightly obscured by data points (TOI-2025b) -- move slightly ?




AO Results:
TOI-1811
SAI-2.5m Speckle by safonov10@gmail.com
BRGamma Palomar by Ciardi

AO Clean!!!



TOI-2025
SAI-2.5m Speckle by safonov10@gmail.com
SPECKLE Clean!



TOi-2145:
ShARCS Ks and J -> Courtney
Palomar Br Gamma - > Ciardi
AO Clean!


TOI-2152:
SAI-2.5m Speckle (3 observations) by safonov10@gmail.com
SPECKLE Shows very faint companion, >5 mags fainter. Could ignore. 




TOI-2154:
SAI-2.5m Speckle (3 observations) by safonov10@gmail.com
SPECKLE Clean!



TOI-2497:
ShARCS Ks and J -> Courtney
SOAR Speckle -> Carl Z.
AO Clean!!!





Old targets:
TOI-2485:
wwSOAR Speckle -> Carl Z.
AO Clean!!!



% TFOP Photometry
TOI-1811:
Excluded:
DSW 05/08/2020 gp
LCO 05/19/2020 B and Z 

TOI-2025:
Excluded:
UW Milwaukee 05/11/2021
HAL LCO 8/1/2020

TOI-2145
Excluded:
LCO McD z 08/13/2020 20210517

TOI-2152
Excluded:
Kourovka 0.4 12102020

TOI-2154
Excluded:
LCO McD 2020 1203 B 


==> fits/All_RVs.tex <==
\begin{deluxetable}{l l l l l}[bt]
\tabletypesize{\scriptsize}
\tablecaption{Relative Radial Velocities for all six systems \label{tab:rv}}
\tablewidth{0pt}
\tablehead{
\colhead{\bjdtdb} & \colhead{RV (m s$^{-1}$)} & \colhead{$\sigma_{RV}$ (m s$^{-1}$)} & Target & \colhead{Instrument}
}
\startdata
2458604.64716 & 193.0 & 43.6 & TOI-628 & TRES \\
2458759.92944 & -1308.2 & 20.4 & TOI-628 & TRES \\
2458769.99526 & -1240.3 & 27.0 & TOI-628 & TRES \\
2458774.95769 &    68.1 & 29.6 & TOI-628 & TRES \\
2458778.98252 &   -66.3 & 24.3 & TOI-628 & TRES \\
2458779.93878 & -1100.2 & 26.0 & TOI-628 & TRES \\
2458782.97523 &  -753.5 & 33.2 & TOI-628 & TRES \\
2458783.98593 & -1304.0 & 27.8 & TOI-628 & TRES \\
2458784.97197 &  -170.1 & 41.7 & TOI-628 & TRES \\
2458785.90368 &  -190.4 & 28.9 & TOI-628 & TRES \\
2458786.96106 & -1263.4 & 23.4 & TOI-628 & TRES \\
2458788.00490 &  -795.9 & 24.1 & TOI-628 & TRES \\
2458742.25270 & 19775.2 & 17.5 & TOI-628 & MINERVA3 \\
2458743.24668 & 19451.6 & 28.8 & TOI-628 & MINERVA3 \\
2458776.20768 & 19913.9 & 20.1 & TOI-628 & MINERVA3 \\
2458776.22945 & 19884.8 & 17.8 & TOI-628 & MINERVA3 \\
2458777.18566 & 19241.9 & 18.6 & TOI-628 & MINERVA3 \\
2458777.20798 & 19277.1 & 16.1 & TOI-628 & MINERVA3 \\
2458794.20339 & 19310.7 & 14.8 & TOI-628 & MINERVA3 \\
2458807.16104 & 19567.8 & 15.3 & TOI-628 & MINERVA3 \\
2458821.15929 & 19287.7 & 14.3 & TOI-628 & MINERVA3 \\
2458742.25270 & 19700.8 & 14.3 & TOI-628 & MINERVA4 \\
2458743.24668 & 19546.3& 30.2 & TOI-628 & MINERVA4 \\
2458776.20768 & 19973.0 & 30.2  & TOI-628 & MINERVA4 \\
2458776.22945 & 19899.2 & 45.3 & TOI-628 & MINERVA4 \\
2458777.18566 & 19179.5 & 21.4 & TOI-628 & MINERVA4 \\
2458777.20798 & 19289.4 & 19.2  & TOI-628 & MINERVA4 \\
2458794.20339 & 19224.7 & 23.4 & TOI-628 & MINERVA4 \\
2458820.18365 & 20160.6 & 22.2 & TOI-628 & MINERVA4 \\
2458820.20505 & 20250.5 & 21.0 & TOI-628 & MINERVA4 \\
2458820.22647 & 20116.1 & 20.4 & TOI-628 & MINERVA4 \\
2458821.15929 & 19297.7 & 20.6 & TOI-628 & MINERVA4 \\
2458742.25270 & 19795.7 & 41.0 & TOI-628 & MINERVA6 \\
2458743.24668 & 19729.6 & 51.2 & TOI-628 & MINERVA6 \\
2458776.20768 & 19895.2 & 33.7 & TOI-628 & MINERVA6 \\
2458776.22945& 19830.7 & 30.0 & TOI-628 & MINERVA6 \\
2458777.18566 & 19400.0 & 33.1 & TOI-628 & MINERVA6 \\
2458777.20798 & 19285.1 & 29.5 & TOI-628 & MINERVA6 \\
2458794.20339 & 19386.1 & 41.6 & TOI-628 & MINERVA6 \\
2458807.16104 & 19713.0 & 38.7 & TOI-628 & MINERVA6 \\
2458820.07662 & 20354.0 & 20.0 & TOI-628 & MINERVA6 \\
2458820.09802 & 20331.1 & 17.0 & TOI-628 & MINERVA6 \\
2458820.11943 & 20328.4 & 18.1 & TOI-628 & MINERVA6 \\
2458820.14084 & 20373.5 & 17.7 & TOI-628 & MINERVA6 \\
2458820.16224 & 20237.8 & 18.1 & TOI-628 & MINERVA6 \\
2458820.18365 & 20263.6 & 19.4 & TOI-628 & MINERVA6 \\
2458820.20505 & 20337.4 & 31.2 & TOI-628 & MINERVA6 \\
2458820.22647 & 20252.0 & 22.1 & TOI-628 & MINERVA6 \\
2458821.15929 & 19404.5 & 17.6 & TOI-628 & MINERVA6 \\
\hline
2458748.89482 & 39168.0 & 29.4 & TOI-640 & CHIRON \\
2458750.90143 & 38985.3 & 12.4 & TOI-640 & CHIRON \\
2458751.90111 & 38972.8 & 43.6 & TOI-640 & CHIRON \\
2458761.89705 & 39044.1 & 15.5 & TOI-640 & CHIRON \\
2458762.88246 & 39122.5 & 12.2 & TOI-640 & CHIRON \\
2458763.89501 & 39123.1 & 26.9 & TOI-640 & CHIRON \\
2458764.86782 & 39083.2 & 18.5 & TOI-640 & CHIRON \\
2458765.87095 & 39030.7 & 10.6 & TOI-640 & CHIRON \\
2458766.87389 & 39084.4 & 13.1 & TOI-640 & CHIRON \\
2458767.84497 & 39128.4 & 32.9 & TOI-640 & CHIRON \\
2458772.85682 & 38967.3 & 68.4 & TOI-640 & CHIRON \\
2458773.86039 & 39170.0 & 15.4 & TOI-640 & CHIRON \\
2458775.84605 & 39014.5 & 30.4 & TOI-640 & CHIRON \\
2458776.87361 & 39054.9 & 12.4 & TOI-640 & CHIRON \\
2458777.81554 & 39182.2 & 12.5 & TOI-640 & CHIRON \\
2458781.86860 & 39000.5 & 14.3 & TOI-640 & CHIRON \\
\hline
2458777.69583 & -50.6 & 48.0 & TOI-1333 & TRES \\
2458779.75728 & 427.0 & 41.9 & TOI-1333 & TRES \\
2458782.59344 & -82.9 & 43.6 & TOI-1333 & TRES \\
2458783.62876 & 156.4 & 35.0 & TOI-1333 & TRES \\
2458784.61463 & 312.2 & 39.4 & TOI-1333 & TRES \\
2458785.66053 & 212.1 & 36.2 & TOI-1333 & TRES \\
2458786.62633 &   9.2 & 40.9 & TOI-1333 & TRES \\
2458787.64417 & -69.9 & 27.8 & TOI-1333 & TRES \\
2458788.74444 & 281.7 & 43.5 & TOI-1333 & TRES \\
2458789.58084 & 294.9 & 30.7 & TOI-1333 & TRES \\
2458790.69847 &  57.1 & 36.1 & TOI-1333 & TRES \\
2458790.71038 &  40.0 & 39.6 & TOI-1333 & TRES \\
2458790.73753 & 112.3 & 43.3 & TOI-1333 & TRES \\
2458790.74582 &  81.2 & 58.2 & TOI-1333 & TRES \\
2458791.67021 & -132.8 & 32.3 & TOI-1333 & TRES \\
2458792.73501 &  63.1 & 35.8 & TOI-1333 & TRES \\
\hline
2458852.80172 & 19374.4 & 21.9 & TOI-1478 & CHIRON \\
2458854.79441 & 19353.2 & 17.0 & TOI-1478 & CHIRON \\
2458857.78705 & 19426.7 & 13.4 & TOI-1478 & CHIRON \\
2458866.57793 & 19330.5 & 18.7 & TOI-1478 & CHIRON \\
2458874.89572 & 19356.5 & 32.3 & TOI-1478 & CHIRON \\
2458876.65005 & 19278.1 & 26.7 & TOI-1478 & CHIRON \\
2458877.71624 & 19385.0 & 15.0 & TOI-1478 & CHIRON \\
2458880.73001 & 19465.4 & 13.1 & TOI-1478 & CHIRON \\
2458884.76504 & 19308.9 & 22.6 & TOI-1478 & CHIRON \\
2458886.72676 & 19363.2 & 16.8 & TOI-1478 & CHIRON \\
2458888.68463 & 19424.8 & 12.5 & TOI-1478 & CHIRON \\
2458890.68066 & 19480.9 & 22.0 & TOI-1478 & CHIRON \\
2458893.71706 & 19344.6 & 22.1 & TOI-1478 & CHIRON \\
2458897.68543 & 19385.4 & 23.2 & TOI-1478 & CHIRON \\
2458899.72093 & 19440.9 & 19.1 & TOI-1478 & CHIRON \\
2458906.65027 & 19323.0 & 20.1 & TOI-1478 & CHIRON \\
2458908.65532 & 19421.0 & 18.7 & TOI-1478 & CHIRON \\
2458910.70128 & 19345.3 & 16.3 & TOI-1478 & CHIRON \\
2458912.63351 & 19405.0 & 15.6 & TOI-1478 & CHIRON \\
2458913.61857 & 19342.8 & 31.9 & TOI-1478 & CHIRON \\
2458914.65319 & 19292.3 & 42.1 & TOI-1478 & CHIRON \\
2458915.67698 & 19323.6 & 20.6 & TOI-1478 & CHIRON \\
2458916.68554 & 19296.5 & 20.1 & TOI-1478 & CHIRON \\
2458917.59662 & 19337.4 & 28.3 & TOI-1478 & CHIRON \\
2458918.59659 & 19361.1 & 19.7 & TOI-1478 & CHIRON \\
2458919.58636 & 19405.6 & 12.2 & TOI-1478 & CHIRON \\
2458920.53375 & 19488.2 & 24.7 & TOI-1478 & CHIRON \\
2458920.55146 & 19499.3 & 22.5 & TOI-1478 & CHIRON \\
2458921.56941 & 19499.8 & 29.8 & TOI-1478 & CHIRON \\
2458922.55123 & 19484.1 & 20.8 & TOI-1478 & CHIRON \\
2458924.54504 & 19327.6 & 25.6 & TOI-1478 & CHIRON \\
\hline
2458875.60994 & 20738.5 & 22.0 & TOI-1478 & CORALIE \\
2458904.63309 & 20764.2 & 19.9 & TOI-1478 & CORALIE \\
2458880.62387 & 20921.4 & 24.3 & TOI-1478 & CORALIE \\
2458886.73153 & 20769.4 & 14.3 & TOI-1478 & CORALIE \\
2458889.64998 & 20884.3 & 18.5 & TOI-1478 & CORALIE \\
2458891.57383 & 20898.3 & 21.3 & TOI-1478 & CORALIE \\
2458894.61978 & 20764.7 & 25.1 & TOI-1478 & CORALIE \\
2458896.61082 & 20772.6 & 26.1 & TOI-1478 & CORALIE \\
2458898.76973 & 20866.5 & 21.8 & TOI-1478 & CORALIE \\
2458900.75324 & 20904.5 & 24.0 & TOI-1478 & CORALIE \\
2458907.58601 & 20812.2 & 16.6 & TOI-1478 & CORALIE \\
2458902.54908 & 20857.2 & 19.2 & TOI-1478 & CORALIE \\
2458918.56928 & 20874.1 & 24.0 & TOI-1478 & CORALIE \\
2458924.57245 & 20795.6 & 13.3 & TOI-1478 & CORALIE \\
\hline
2458910.73537 & 20910.3 & 7.5 & TOI-1478 & FEROS \\
2458915.72299 & 20733.1 & 7.5 & TOI-1478 & FEROS \\
2458921.59907 & 20909.4 & 10.5 & TOI-1478 & FEROS \\
2458925.63513 & 20739.6 & 7.2 & TOI-1478 & FEROS \\
2458927.57429 & 20788.7 & 7.0 & TOI-1478 & FEROS \\
2458928.61419 & 20825.5 & 6.4 & TOI-1478 & FEROS \\
2458929.59990 & 20860.3 & 6.4 & TOI-1478 & FEROS \\
2458930.61647 & 20884.6 & 8.2 & TOI-1478 & FEROS \\
\hline
2458829.86525 & 67.4 & 27.6 & TOI-1478 & TRES \\
2458833.96527 & -193.2 & 24.1 & TOI-1478 & TRES \\
2458912.81019 & -35.8 & 31.5 & TOI-1478 & TRES \\
2458913.76762 & -30.3 & 27.2 & TOI-1478 & TRES \\
2458915.67646 & -105.1 & 29.8 & TOI-1478 & TRES \\
2458923.76794 & -60.6 & 26.5 & TOI-1478 & TRES \\
2458924.70977 & -104.8 & 24.1 & TOI-1478 & TRES \\
2459144.01566 & 116.0 & 19.9 & TOI-1478 & TRES \\
\hline
2458847.77575 & -184.1 & 32.0 & TOI-1601 & TRES\\
2458851.79762 & -35.8 & 33.0 & TOI-1601 & TRES\\
2458871.66744 & -13.0 & 30.3 & TOI-1601 & TRES\\
2458887.69829 & -5.2 & 37.3 & TOI-1601 & TRES\\
2458888.65050 & -41.4 & 24.9 & TOI-1601 & TRES\\
2458892.64702 & -18.6 & 25.7 & TOI-1601 & TRES\\
2458895.62280 & -198.4 & 29.2 & TOI-1601 & TRES\\
2458900.66400 & -201.6 & 30.3 & TOI-1601 & TRES\\
2458908.67094 & -103.1 & 38.3 & TOI-1601 & TRES\\
2458913.62964 & -68.2 & 26.6 & TOI-1601 & TRES\\
2458914.62865 & -9.1 & 37.8 & TOI-1601 & TRES\\
2459044.97455 & -223.0 & 31.5 & TOI-1601 & TRES\\
2459056.95754 & -114.3 & 28.8 & TOI-1601 & TRES\\
2459057.97099 & -61.2 & 35.0 & TOI-1601 & TRES\\
2459058.97480 & -44.0 & 35.2 & TOI-1601 & TRES\\
2459060.97114 & -147.6 & 32.6 & TOI-1601 & TRES\\
2459061.98117 & -125.2 & 31.7 & TOI-1601 & TRES\\
\hline
\enddata
\end{deluxetable}

==> fits/authors.tex <==
%\correspondingauthor{Joseph E. Rodriguez} 
%\email{jrod@msu.edu}
%
\author[0000-0001-8812-0565]{Joseph E. Rodriguez} %agreed
\affiliation{\msu}

\author[0000-0002-8964-8377]{Samuel N. Quinn} %agreed
\affiliation{\cfa}

\author[0000-0001-7246-5438]{Andrew Vanderburg} %agreed
\affiliation{\MIT}

\author[0000-0002-4891-3517]{George Zhou} %agreed
\affiliation{\cfa}

\author[0000-0003-3773-5142]{Jason D. Eastman}  %agreed
\affiliation{\cfa}

\author[0000-0002-9165-6245]{Erica Thygesen} %agreed
\affiliation{\msu}

\author[0000-0001-6279-0595]{Bryson Cale}%MINERVA
\affiliation{\gmu}

\author[0000-0002-5741-3047]{David R. Ciardi}  %AO All
\affiliation{\nexsci}

\author[0000-0002-5005-1215]{Phillip A.\ Reed} %SG1 obs %agreed
\affiliation{\Kutztown}

\author[0000-0001-6588-9574]{Karen A.\ Collins}%TFOP %agreed
\affiliation{\cfa}

\author[0000-0002-0582-1751]{Ryan J. Oelkers} %KELT
\affiliation{\txammul}

\author[0000-0001-6637-5401]{Allyson Bieryla} % KepCam and TRES %agreed
\affiliation{\cfa}

\author[0000-0001-9911-7388]{David W. Latham} % TRES %agreed
\affiliation{\cfa}

\author[0000-0002-9329-2190]{Erica J.\ Gonzales} %AO leader
\nsf
\affiliation{\ucsc}

\author{Coel Hellier} %WASP
\affiliation{\keele}

\author[0000-0003-0395-9869]{B. Scott Gaudi} % KELT/UVW Analysis
\affiliation{\osu}

\author{Kirill Sokolovsky} %agreed
\affiliation{\msu}

\author[0000-0002-7382-0160]{Jack Schulte} %agreed
\affiliation{\msu}

\author{Gregor Srdoc}
\affiliation{\Kotizarovci}

\author[0000-0003-0497-2651]{John Kielkopf}% SG1
\affiliation{\louisville}

\author[0000-0001-9927-7269]{Ferran Grau Horta} %SG1
\affiliation{\calou}

\author[0000-0001-8879-7138]{Bob Massey} %SG1 
\affiliation{\Villa}

\author[0000-0002-5674-2404]{Phil Evans} %SG1
\affiliation{\ElSauce}

\author[0000-0003-4658-7567]{Denise C. Stephens} %Sg1 BYU
\affiliation{\byu}

\author[0000-0001-9504-1486]{Kim K.\ McLeod} %SG1 LCO
\affiliation{\wellesley}

\author[0000-0002-4070-7831]{Nikita Chazov}
\affiliation{\Ural}

\author[0000-0001-9388-691X]{Vadim Krushinsky}
\affiliation{\Ural}

\author{Mourad Ghachoui}
\affiliation{\Oikaimeden}
\affiliation{\liegeastrobio}

\author{Boris Safonov} %Speckle
\affiliation{\Sternberg}

\author[0000-0001-9408-8848]{Cayla M. Dedrick} % MINERVA
\affiliation{\psu}
\affiliation{\psust}

\author{George R. Ricker} % Architect Agreed
\affiliation{\MIT}

\author{Roland K. Vanderspek}% Architect
\affiliation{\MIT}

\author[0000-0002-6892-6948]{Sara Seager}% Architect
\affiliation{\MIT}
\affiliation{\MITEPS}
\affiliation{\MITAA}

\author[0000-0002-4265-047X]{Joshua N. Winn} % Architect
\affiliation{\princeton}

\author[0000-0002-4715-9460]{Jon M. Jenkins}% Architect
\affiliation{\ames}


%Alphabetized:
\author{Owen Alfaro} %jwittroc@gmu.edu
\affiliation{\gmu}

\author[0000-0001-7416-7522]{D. R. Anderson}%WASP
\affiliation{\keele}
\affiliation{\warwick}

\author{Elias Ayad} %SG1 MSU
\affiliation{\msu}

\author[0000-0002-9539-4203]{Thomas G.\ Beatty} %KELT
\affiliation{\steward}

\author{Alexandr A. Belinsky} %SPECKLE
\affiliation{\Sternberg}

\author{Zouhair Benkhaldoun}% SG1 OWL
\affiliation{\Oikaimeden}

\author{Perry Berlind} %TRES Agreed
\affiliation{\cfa}

\author[0000-0002-6096-1749]{Cullen H. Blake} % Confirmed
\affiliation{\UPenn}

\author{Michael J. Bowen} %SG! GMU
\affiliation{\gmu}

\author[0000-0001-6037-2971]{Andrew W. Boyle}  %AO All
\affiliation{\nexsci}

\author{Dalton Branson} % Confirmed
\affiliation{\montana}


\author[0000-0002-2830-5661]{Michael L. Calkins} %TRES agreed
\affiliation{\cfa}

\author{Emma Campbell} %Sg1 BYU
\affiliation{\byu}

\author{Laura Chomiuk} %SG1 MSU
\affiliation{\msu}

\author[0000-0003-2781-3207]{Kevin I. Collins} %SG1 GMU
\affiliation{\gmu}

\author[0000-0003-1012-4771]{Matthew A. Cornachione} % Confirmed
\affiliation{\utah}


\author[0000-0002-9789-5474]{Gilbert A. Esquerdo} %TRES
\affiliation{\cfa}

\author[0000-0002-2457-7889]{Dax L. Feliz}%KELT
\affiliation{\vanderbilt}

\author{Akihiko Fukui}
\affiliation{\iac}
\affiliation{\Subaru}
\affiliation{\SOKENDAI}

\author[0000-0002-4503-9705]{Tianjun Gan}
\affil{\Tsinghua}

\author{Maria V. Goliguzova} %SPECKLE
\affiliation{\Sternberg}

\author[0000-0002-1321-3174]{Jarrod Hansen} %Sg1 BYU
\affiliation{\byu}

\author[0000-0002-9867-7938]{Eric G. Hintz} %Sg1 BYU
\affiliation{\byu}


\author[0000-0003-0918-7484]{Chelsea X. Huang} %agreed
\torres
\affiliation{\MIT}

\author[0000-0001-5160-4486]{David J. James} %KELT
\affiliation{\ASTRAVEO}

\author{Jacob S. Jensen} %Sg1 BYU
\affiliation{\byu}

\author[0000-0001-9397-4768]{Samson A. Johnson} % Confirmed
\affiliation{\osu}

\author{Barkaoui Khalid}
\affiliation{\liegeastrobio}
\affiliation{\MITEPS}
\affiliation{\iac}

\author{Myung-Jin Kim}
\affiliation{\KASSI}

\author[0000-0002-4236-9020]{Rudolf B. Kuhn} %KELT 
\affiliation{\saao}
\affiliation{\salt}

\author[0000-0003-2527-1598]{Michael B. Lund}% KELT AO
\affiliation{\nexsci}

\author[0000-0002-8041-1832]{Nate McCrady} % Confirmed
\affiliation{\montana}


\author[0000-0003-3594-1823]{Jessica Mink}%TRES
\affiliation{\cfa}

\author{Felipe Murgas}
\affiliation{\SOKENDAI}
\affiliation{\lalaguna}

\author{Lauren Murphy} %SG1 obs %agreed
\affiliation{\Kutztown}

\author[0000-0001-8511-2981]{Norio Narita}
\affiliation{\astrobiojapan}
\affiliation{\jstpresto}
\affiliation{\naoj}
\affiliation{\iac}

\author{Patrick Newman}
\affiliation{\gmu}

\author[0000-0002-3827-8417]{Joshua Pepper}%KELT Agreed
\affiliation{\lehigh}

\author[0000-0002-8864-1667]{Peter Plavchan} % Confirmed
\affiliation{\gmu}

\author[0000-0002-2007-2461]{Alexander A. Popov}
\affiliation{\Ural}

\author[0000-0003-2935-7196]{Markus Rabus}
\affiliation{\lco}
\affiliation{\ucsb}
\affiliation{\ucscchile}

\author{Jessica Ranshaw} 
\affiliation{\msu}

\author{Jennifer Rodriguez}
\affiliation{\msu}

\author{Dong-Goo Roh}
\affiliation{\KASSI}

\author{Michael A Reefe}% mreefe@gmu.edu
\affiliation{\gmu}


\author[0000-0001-5016-3359]{Robert J.\ Siverd} %KELT
\affiliation{\gemini}

\author{David H. Sliski} % Confirmed
\affiliation{\UPenn}

\author[0000-0002-3481-9052]{Keivan G. Stassun} %KELT %agreed
\affiliation{\vanderbilt}
\affiliation{\fisk}

\author[0000-0002-5951-8328]{Daniel J.\ Stevens} %KELT
\eberly
\affiliation{\psu}
\affiliation{\psust}

\author{Abderahmane Soubkiou}% SG1 OWL
\affiliation{\Oikaimeden}
\affiliation{\CAUP}
\affiliation{\Faculdade}

\author{Noah Vowell} 
\affiliation{\msu}

\author{Payton Walton}
\affiliation{\msu}

\author{R. G. West}%WASP
\affiliation{\warwick}
\affiliation{\warwickceh}

\author[0000-0003-1928-0578]{Maurice L. Wilson} % Confirmed
\affiliation{\cfa}


\author[0000-0001-9957-9304]{Robert A. Wittenmyer} % Confirmed
\affiliation{\usq}


\author{Justin Michael William Wittrock} %jwittroc@gmu.edu
\affiliation{\gmu}

\author{Shania Wolf}%CFRACO reduction
\affiliation{\lehigh}

\author[0000-0001-6160-5888]{Jason T. Wright}
\affiliation{\psu}
\affiliation{\psust}

\author{Hong-Suh Yim}
\affiliation{\KASSI}

\author{Evan Zobel} 
\affiliation{\msu}



%%%%%%%%%%%%%%%%%% MINERVA Authors %%%%%%%%%%%%%%%%%%%%%%
%\author[0000-0001-6279-0595]{Bryson Cale} % major RV contribution -- confirmed
%\affiliation{\gmu} 

%\author[0000-0001-9408-8848]{Cayla M. Dedrick} % major operational contribution -- confirmed
%\affiliation{\psu}
%\affiliation{\psust}

%\author[0000-0003-3773-5142]{Jason D.\ Eastman} % confirmed
%\affiliation{\cfa} 

% begin MINERVA alphabetical



%\author[0000-0002-1704-6289]{John Asher Johnson} 
%\affiliation{\cfa}



%%%%%%%%%%%%%%%%%% End MINERVA Authors %%%%%%%%%%%%%%%%%%%


==> fits/defs.tex <==
\newcommand{\mvalone}{\ensuremath{0.974^{+0.061}_{-0.055}}}
\newcommand{\mvaltwo}{\ensuremath{0.974^{+0.061}_{-0.055}}}
\newcommand{\mvalthree}{\ensuremath{0.974^{+0.061}_{-0.055}}}
\newcommand{\mvalfour}{\ensuremath{0.974^{+0.061}_{-0.055}}}
\newcommand{\mvalfive}{\ensuremath{0.974^{+0.061}_{-0.055}}}
\newcommand{\mvalsix}{\ensuremath{0.974^{+0.061}_{-0.055}}}
\newcommand{\rvalone}{\ensuremath{1.022^{+0.029}_{-0.028}}}
\newcommand{\rvaltwo}{\ensuremath{1.022^{+0.029}_{-0.028}}}
\newcommand{\rvalthree}{\ensuremath{1.022^{+0.029}_{-0.028}}}
\newcommand{\rvalfour}{\ensuremath{1.022^{+0.029}_{-0.028}}}
\newcommand{\rvalfive}{\ensuremath{1.022^{+0.029}_{-0.028}}}
\newcommand{\rvalsix}{\ensuremath{1.022^{+0.029}_{-0.028}}}
\newcommand{\rstarsedvalone}{\ensuremath{1.0120^{+0.010}_{-0.0099}}}
\newcommand{\rstarsedvaltwo}{\ensuremath{1.0120^{+0.010}_{-0.0099}}}
\newcommand{\rstarsedvalthree}{\ensuremath{1.0120^{+0.010}_{-0.0099}}}
\newcommand{\rstarsedvalfour}{\ensuremath{1.0120^{+0.010}_{-0.0099}}}
\newcommand{\rstarsedvalfive}{\ensuremath{1.0120^{+0.010}_{-0.0099}}}
\newcommand{\rstarsedvalsix}{\ensuremath{1.0120^{+0.010}_{-0.0099}}}
\newcommand{\lvalone}{\ensuremath{0.953^{+0.036}_{-0.034}}}
\newcommand{\lvaltwo}{\ensuremath{0.953^{+0.036}_{-0.034}}}
\newcommand{\lvalthree}{\ensuremath{0.953^{+0.036}_{-0.034}}}
\newcommand{\lvalfour}{\ensuremath{0.953^{+0.036}_{-0.034}}}
\newcommand{\lvalfive}{\ensuremath{0.953^{+0.036}_{-0.034}}}
\newcommand{\lvalsix}{\ensuremath{0.953^{+0.036}_{-0.034}}}
\newcommand{\fbolvalone}{\ensuremath{0.000000001325^{+0.000000000045}_{-0.000000000044}}}
\newcommand{\fbolvaltwo}{\ensuremath{0.000000001325^{+0.000000000045}_{-0.000000000044}}}
\newcommand{\fbolvalthree}{\ensuremath{0.000000001325^{+0.000000000045}_{-0.000000000044}}}
\newcommand{\fbolvalfour}{\ensuremath{0.000000001325^{+0.000000000045}_{-0.000000000044}}}
\newcommand{\fbolvalfive}{\ensuremath{0.000000001325^{+0.000000000045}_{-0.000000000044}}}
\newcommand{\fbolvalsix}{\ensuremath{0.000000001325^{+0.000000000045}_{-0.000000000044}}}
\newcommand{\fehovalone}{\ensuremath{1.29^{+0.15}_{-0.13}}}
\newcommand{\fehovaltwo}{\ensuremath{1.29^{+0.15}_{-0.13}}}
\newcommand{\fehovalthree}{\ensuremath{1.29^{+0.15}_{-0.13}}}
\newcommand{\fehovalfour}{\ensuremath{1.29^{+0.15}_{-0.13}}}
\newcommand{\fehovalfive}{\ensuremath{1.29^{+0.15}_{-0.13}}}
\newcommand{\fehovalsix}{\ensuremath{1.29^{+0.15}_{-0.13}}}
\newcommand{\loggvalone}{\ensuremath{4.408^{+0.040}_{-0.038}}}
\newcommand{\loggvaltwo}{\ensuremath{4.408^{+0.040}_{-0.038}}}
\newcommand{\loggvalthree}{\ensuremath{4.408^{+0.040}_{-0.038}}}
\newcommand{\loggvalfour}{\ensuremath{4.408^{+0.040}_{-0.038}}}
\newcommand{\loggvalfive}{\ensuremath{4.408^{+0.040}_{-0.038}}}
\newcommand{\loggvalsix}{\ensuremath{4.408^{+0.040}_{-0.038}}}
\newcommand{\tfehvalone}{\ensuremath{5641^{+83}_{-82}}}
\newcommand{\tfehvaltwo}{\ensuremath{5641^{+83}_{-82}}}
\newcommand{\tfehvalthree}{\ensuremath{5641^{+83}_{-82}}}
\newcommand{\tfehvalfour}{\ensuremath{5641^{+83}_{-82}}}
\newcommand{\tfehvalfive}{\ensuremath{5641^{+83}_{-82}}}
\newcommand{\tfehvalsix}{\ensuremath{5641^{+83}_{-82}}}
\newcommand{\tfehsedvalone}{\ensuremath{5670^{+49}_{-52}}}
\newcommand{\tfehsedvaltwo}{\ensuremath{5670^{+49}_{-52}}}
\newcommand{\tfehsedvalthree}{\ensuremath{5670^{+49}_{-52}}}
\newcommand{\tfehsedvalfour}{\ensuremath{5670^{+49}_{-52}}}
\newcommand{\tfehsedvalfive}{\ensuremath{5670^{+49}_{-52}}}
\newcommand{\tfehsedvalsix}{\ensuremath{5670^{+49}_{-52}}}
\newcommand{\fehffehhvalone}{\ensuremath{0.092^{+0.070}_{-0.066}}}
\newcommand{\fehffehhvaltwo}{\ensuremath{0.092^{+0.070}_{-0.066}}}
\newcommand{\fehffehhvalthree}{\ensuremath{0.092^{+0.070}_{-0.066}}}
\newcommand{\fehffehhvalfour}{\ensuremath{0.092^{+0.070}_{-0.066}}}
\newcommand{\fehffehhvalfive}{\ensuremath{0.092^{+0.070}_{-0.066}}}
\newcommand{\fehffehhvalsix}{\ensuremath{0.092^{+0.070}_{-0.066}}}
\newcommand{\fehffehhfehzerovalone}{\ensuremath{0.110^{+0.068}_{-0.064}}}
\newcommand{\fehffehhfehzerovaltwo}{\ensuremath{0.110^{+0.068}_{-0.064}}}
\newcommand{\fehffehhfehzerovalthree}{\ensuremath{0.110^{+0.068}_{-0.064}}}
\newcommand{\fehffehhfehzerovalfour}{\ensuremath{0.110^{+0.068}_{-0.064}}}
\newcommand{\fehffehhfehzerovalfive}{\ensuremath{0.110^{+0.068}_{-0.064}}}
\newcommand{\fehffehhfehzerovalsix}{\ensuremath{0.110^{+0.068}_{-0.064}}}
\newcommand{\agvalone}{\ensuremath{6.7^{+4.1}_{-3.8}}}
\newcommand{\agvaltwo}{\ensuremath{6.7^{+4.1}_{-3.8}}}
\newcommand{\agvalthree}{\ensuremath{6.7^{+4.1}_{-3.8}}}
\newcommand{\agvalfour}{\ensuremath{6.7^{+4.1}_{-3.8}}}
\newcommand{\agvalfive}{\ensuremath{6.7^{+4.1}_{-3.8}}}
\newcommand{\agvalsix}{\ensuremath{6.7^{+4.1}_{-3.8}}}
\newcommand{\eepvalone}{\ensuremath{377^{+30}_{-37}}}
\newcommand{\eepvaltwo}{\ensuremath{377^{+30}_{-37}}}
\newcommand{\eepvalthree}{\ensuremath{377^{+30}_{-37}}}
\newcommand{\eepvalfour}{\ensuremath{377^{+30}_{-37}}}
\newcommand{\eepvalfive}{\ensuremath{377^{+30}_{-37}}}
\newcommand{\eepvalsix}{\ensuremath{377^{+30}_{-37}}}
\newcommand{\avvalone}{\ensuremath{0.064^{+0.038}_{-0.042}}}
\newcommand{\avvaltwo}{\ensuremath{0.064^{+0.038}_{-0.042}}}
\newcommand{\avvalthree}{\ensuremath{0.064^{+0.038}_{-0.042}}}
\newcommand{\avvalfour}{\ensuremath{0.064^{+0.038}_{-0.042}}}
\newcommand{\avvalfive}{\ensuremath{0.064^{+0.038}_{-0.042}}}
\newcommand{\avvalsix}{\ensuremath{0.064^{+0.038}_{-0.042}}}
\newcommand{\sigfehasedvalone}{\ensuremath{0.73^{+0.24}_{-0.16}}}
\newcommand{\sigfehasedvaltwo}{\ensuremath{0.73^{+0.24}_{-0.16}}}
\newcommand{\sigfehasedvalthree}{\ensuremath{0.73^{+0.24}_{-0.16}}}
\newcommand{\sigfehasedvalfour}{\ensuremath{0.73^{+0.24}_{-0.16}}}
\newcommand{\sigfehasedvalfive}{\ensuremath{0.73^{+0.24}_{-0.16}}}
\newcommand{\sigfehasedvalsix}{\ensuremath{0.73^{+0.24}_{-0.16}}}
\newcommand{\vafehpivalone}{\ensuremath{6.594^{+0.050}_{-0.051}}}
\newcommand{\vafehpivaltwo}{\ensuremath{6.594^{+0.050}_{-0.051}}}
\newcommand{\vafehpivalthree}{\ensuremath{6.594^{+0.050}_{-0.051}}}
\newcommand{\vafehpivalfour}{\ensuremath{6.594^{+0.050}_{-0.051}}}
\newcommand{\vafehpivalfive}{\ensuremath{6.594^{+0.050}_{-0.051}}}
\newcommand{\vafehpivalsix}{\ensuremath{6.594^{+0.050}_{-0.051}}}
\newcommand{\dvalone}{\ensuremath{151.7^{+1.2}_{-1.1}}}
\newcommand{\dvaltwo}{\ensuremath{151.7^{+1.2}_{-1.1}}}
\newcommand{\dvalthree}{\ensuremath{151.7^{+1.2}_{-1.1}}}
\newcommand{\dvalfour}{\ensuremath{151.7^{+1.2}_{-1.1}}}
\newcommand{\dvalfive}{\ensuremath{151.7^{+1.2}_{-1.1}}}
\newcommand{\dvalsix}{\ensuremath{151.7^{+1.2}_{-1.1}}}
\newcommand{\pvalone}{\ensuremath{10.180202\pm0.000026}}
\newcommand{\pvaltwo}{\ensuremath{10.180202\pm0.000026}}
\newcommand{\pvalthree}{\ensuremath{10.180202\pm0.000026}}
\newcommand{\pvalfour}{\ensuremath{10.180202\pm0.000026}}
\newcommand{\pvalfive}{\ensuremath{10.180202\pm0.000026}}
\newcommand{\pvalsix}{\ensuremath{10.180202\pm0.000026}}
\newcommand{\rpvalone}{\ensuremath{1.009^{+0.039}_{-0.035}}}
\newcommand{\rpvaltwo}{\ensuremath{1.009^{+0.039}_{-0.035}}}
\newcommand{\rpvalthree}{\ensuremath{1.009^{+0.039}_{-0.035}}}
\newcommand{\rpvalfour}{\ensuremath{1.009^{+0.039}_{-0.035}}}
\newcommand{\rpvalfive}{\ensuremath{1.009^{+0.039}_{-0.035}}}
\newcommand{\rpvalsix}{\ensuremath{1.009^{+0.039}_{-0.035}}}
\newcommand{\mpvalone}{\ensuremath{0.847^{+0.052}_{-0.049}}}
\newcommand{\mpvaltwo}{\ensuremath{0.847^{+0.052}_{-0.049}}}
\newcommand{\mpvalthree}{\ensuremath{0.847^{+0.052}_{-0.049}}}
\newcommand{\mpvalfour}{\ensuremath{0.847^{+0.052}_{-0.049}}}
\newcommand{\mpvalfive}{\ensuremath{0.847^{+0.052}_{-0.049}}}
\newcommand{\mpvalsix}{\ensuremath{0.847^{+0.052}_{-0.049}}}
\newcommand{\tcvalone}{\ensuremath{2458495.92607^{+0.00043}_{-0.00042}}}
\newcommand{\tcvaltwo}{\ensuremath{2458495.92607^{+0.00043}_{-0.00042}}}
\newcommand{\tcvalthree}{\ensuremath{2458495.92607^{+0.00043}_{-0.00042}}}
\newcommand{\tcvalfour}{\ensuremath{2458495.92607^{+0.00043}_{-0.00042}}}
\newcommand{\tcvalfive}{\ensuremath{2458495.92607^{+0.00043}_{-0.00042}}}
\newcommand{\tcvalsix}{\ensuremath{2458495.92607^{+0.00043}_{-0.00042}}}
\newcommand{\ttvalone}{\ensuremath{2458495.92607^{+0.00043}_{-0.00042}}}
\newcommand{\ttvaltwo}{\ensuremath{2458495.92607^{+0.00043}_{-0.00042}}}
\newcommand{\ttvalthree}{\ensuremath{2458495.92607^{+0.00043}_{-0.00042}}}
\newcommand{\ttvalfour}{\ensuremath{2458495.92607^{+0.00043}_{-0.00042}}}
\newcommand{\ttvalfive}{\ensuremath{2458495.92607^{+0.00043}_{-0.00042}}}
\newcommand{\ttvalsix}{\ensuremath{2458495.92607^{+0.00043}_{-0.00042}}}
\newcommand{\tzerovalone}{\ensuremath{2458587.54789\pm0.00036}}
\newcommand{\tzerovaltwo}{\ensuremath{2458587.54789\pm0.00036}}
\newcommand{\tzerovalthree}{\ensuremath{2458587.54789\pm0.00036}}
\newcommand{\tzerovalfour}{\ensuremath{2458587.54789\pm0.00036}}
\newcommand{\tzerovalfive}{\ensuremath{2458587.54789\pm0.00036}}
\newcommand{\tzerovalsix}{\ensuremath{2458587.54789\pm0.00036}}
\newcommand{\avalone}{\ensuremath{0.0911^{+0.0019}_{-0.0017}}}
\newcommand{\avaltwo}{\ensuremath{0.0911^{+0.0019}_{-0.0017}}}
\newcommand{\avalthree}{\ensuremath{0.0911^{+0.0019}_{-0.0017}}}
\newcommand{\avalfour}{\ensuremath{0.0911^{+0.0019}_{-0.0017}}}
\newcommand{\avalfive}{\ensuremath{0.0911^{+0.0019}_{-0.0017}}}
\newcommand{\avalsix}{\ensuremath{0.0911^{+0.0019}_{-0.0017}}}
\newcommand{\ivalone}{\ensuremath{88.85^{+0.57}_{-0.34}}}
\newcommand{\ivaltwo}{\ensuremath{88.85^{+0.57}_{-0.34}}}
\newcommand{\ivalthree}{\ensuremath{88.85^{+0.57}_{-0.34}}}
\newcommand{\ivalfour}{\ensuremath{88.85^{+0.57}_{-0.34}}}
\newcommand{\ivalfive}{\ensuremath{88.85^{+0.57}_{-0.34}}}
\newcommand{\ivalsix}{\ensuremath{88.85^{+0.57}_{-0.34}}}
\newcommand{\valone}{\ensuremath{0.047^{+0.054}_{-0.034}}}
\newcommand{\valtwo}{\ensuremath{0.047^{+0.054}_{-0.034}}}
\newcommand{\valthree}{\ensuremath{0.047^{+0.054}_{-0.034}}}
\newcommand{\valfour}{\ensuremath{0.047^{+0.054}_{-0.034}}}
\newcommand{\valfive}{\ensuremath{0.047^{+0.054}_{-0.034}}}
\newcommand{\valsix}{\ensuremath{0.047^{+0.054}_{-0.034}}}
\newcommand{\ofehgavalone}{\ensuremath{85^{+44}_{-47}}}
\newcommand{\ofehgavaltwo}{\ensuremath{85^{+44}_{-47}}}
\newcommand{\ofehgavalthree}{\ensuremath{85^{+44}_{-47}}}
\newcommand{\ofehgavalfour}{\ensuremath{85^{+44}_{-47}}}
\newcommand{\ofehgavalfive}{\ensuremath{85^{+44}_{-47}}}
\newcommand{\ofehgavalsix}{\ensuremath{85^{+44}_{-47}}}
\newcommand{\tfehqvalone}{\ensuremath{910\pm11}}
\newcommand{\tfehqvaltwo}{\ensuremath{910\pm11}}
\newcommand{\tfehqvalthree}{\ensuremath{910\pm11}}
\newcommand{\tfehqvalfour}{\ensuremath{910\pm11}}
\newcommand{\tfehqvalfive}{\ensuremath{910\pm11}}
\newcommand{\tfehqvalsix}{\ensuremath{910\pm11}}
\newcommand{\fehaufehcifehcvalone}{\ensuremath{53^{+14}_{-11}}}
\newcommand{\fehaufehcifehcvaltwo}{\ensuremath{53^{+14}_{-11}}}
\newcommand{\fehaufehcifehcvalthree}{\ensuremath{53^{+14}_{-11}}}
\newcommand{\fehaufehcifehcvalfour}{\ensuremath{53^{+14}_{-11}}}
\newcommand{\fehaufehcifehcvalfive}{\ensuremath{53^{+14}_{-11}}}
\newcommand{\fehaufehcifehcvalsix}{\ensuremath{53^{+14}_{-11}}}
\newcommand{\kvalone}{\ensuremath{81.0^{+3.8}_{-4.0}}}
\newcommand{\kvaltwo}{\ensuremath{81.0^{+3.8}_{-4.0}}}
\newcommand{\kvalthree}{\ensuremath{81.0^{+3.8}_{-4.0}}}
\newcommand{\kvalfour}{\ensuremath{81.0^{+3.8}_{-4.0}}}
\newcommand{\kvalfive}{\ensuremath{81.0^{+3.8}_{-4.0}}}
\newcommand{\kvalsix}{\ensuremath{81.0^{+3.8}_{-4.0}}}
\newcommand{\rprvalone}{\ensuremath{0.1016^{+0.0017}_{-0.0016}}}
\newcommand{\rprvaltwo}{\ensuremath{0.1016^{+0.0017}_{-0.0016}}}
\newcommand{\rprvalthree}{\ensuremath{0.1016^{+0.0017}_{-0.0016}}}
\newcommand{\rprvalfour}{\ensuremath{0.1016^{+0.0017}_{-0.0016}}}
\newcommand{\rprvalfive}{\ensuremath{0.1016^{+0.0017}_{-0.0016}}}
\newcommand{\rprvalsix}{\ensuremath{0.1016^{+0.0017}_{-0.0016}}}
\newcommand{\arvalone}{\ensuremath{19.19^{+0.73}_{-0.69}}}
\newcommand{\arvaltwo}{\ensuremath{19.19^{+0.73}_{-0.69}}}
\newcommand{\arvalthree}{\ensuremath{19.19^{+0.73}_{-0.69}}}
\newcommand{\arvalfour}{\ensuremath{19.19^{+0.73}_{-0.69}}}
\newcommand{\arvalfive}{\ensuremath{19.19^{+0.73}_{-0.69}}}
\newcommand{\arvalsix}{\ensuremath{19.19^{+0.73}_{-0.69}}}
\newcommand{\dfehlfehavalone}{\ensuremath{0.01032^{+0.00035}_{-0.00032}}}
\newcommand{\dfehlfehavaltwo}{\ensuremath{0.01032^{+0.00035}_{-0.00032}}}
\newcommand{\dfehlfehavalthree}{\ensuremath{0.01032^{+0.00035}_{-0.00032}}}
\newcommand{\dfehlfehavalfour}{\ensuremath{0.01032^{+0.00035}_{-0.00032}}}
\newcommand{\dfehlfehavalfive}{\ensuremath{0.01032^{+0.00035}_{-0.00032}}}
\newcommand{\dfehlfehavalsix}{\ensuremath{0.01032^{+0.00035}_{-0.00032}}}
\newcommand{\dfehpvalone}{\ensuremath{0.01032^{+0.00035}_{-0.00032}}}
\newcommand{\dfehpvaltwo}{\ensuremath{0.01032^{+0.00035}_{-0.00032}}}
\newcommand{\dfehpvalthree}{\ensuremath{0.01032^{+0.00035}_{-0.00032}}}
\newcommand{\dfehpvalfour}{\ensuremath{0.01032^{+0.00035}_{-0.00032}}}
\newcommand{\dfehpvalfive}{\ensuremath{0.01032^{+0.00035}_{-0.00032}}}
\newcommand{\dfehpvalsix}{\ensuremath{0.01032^{+0.00035}_{-0.00032}}}
\newcommand{\fehauvalone}{\ensuremath{0.0177^{+0.0025}_{-0.0021}}}
\newcommand{\fehauvaltwo}{\ensuremath{0.0177^{+0.0025}_{-0.0021}}}
\newcommand{\fehauvalthree}{\ensuremath{0.0177^{+0.0025}_{-0.0021}}}
\newcommand{\fehauvalfour}{\ensuremath{0.0177^{+0.0025}_{-0.0021}}}
\newcommand{\fehauvalfive}{\ensuremath{0.0177^{+0.0025}_{-0.0021}}}
\newcommand{\fehauvalsix}{\ensuremath{0.0177^{+0.0025}_{-0.0021}}}
\newcommand{\tonefourvalone}{\ensuremath{0.1673^{+0.0024}_{-0.0021}}}
\newcommand{\tonefourvaltwo}{\ensuremath{0.1673^{+0.0024}_{-0.0021}}}
\newcommand{\tonefourvalthree}{\ensuremath{0.1673^{+0.0024}_{-0.0021}}}
\newcommand{\tonefourvalfour}{\ensuremath{0.1673^{+0.0024}_{-0.0021}}}
\newcommand{\tonefourvalfive}{\ensuremath{0.1673^{+0.0024}_{-0.0021}}}
\newcommand{\tonefourvalsix}{\ensuremath{0.1673^{+0.0024}_{-0.0021}}}
\newcommand{\tfwhmvalone}{\ensuremath{0.1495\pm0.0011}}
\newcommand{\tfwhmvaltwo}{\ensuremath{0.1495\pm0.0011}}
\newcommand{\tfwhmvalthree}{\ensuremath{0.1495\pm0.0011}}
\newcommand{\tfwhmvalfour}{\ensuremath{0.1495\pm0.0011}}
\newcommand{\tfwhmvalfive}{\ensuremath{0.1495\pm0.0011}}
\newcommand{\tfwhmvalsix}{\ensuremath{0.1495\pm0.0011}}
\newcommand{\bvalone}{\ensuremath{0.37^{+0.11}_{-0.19}}}
\newcommand{\bvaltwo}{\ensuremath{0.37^{+0.11}_{-0.19}}}
\newcommand{\bvalthree}{\ensuremath{0.37^{+0.11}_{-0.19}}}
\newcommand{\bvalfour}{\ensuremath{0.37^{+0.11}_{-0.19}}}
\newcommand{\bvalfive}{\ensuremath{0.37^{+0.11}_{-0.19}}}
\newcommand{\bvalsix}{\ensuremath{0.37^{+0.11}_{-0.19}}}
\newcommand{\bsvalone}{\ensuremath{0.400^{+0.093}_{-0.19}}}
\newcommand{\bsvaltwo}{\ensuremath{0.400^{+0.093}_{-0.19}}}
\newcommand{\bsvalthree}{\ensuremath{0.400^{+0.093}_{-0.19}}}
\newcommand{\bsvalfour}{\ensuremath{0.400^{+0.093}_{-0.19}}}
\newcommand{\bsvalfive}{\ensuremath{0.400^{+0.093}_{-0.19}}}
\newcommand{\bsvalsix}{\ensuremath{0.400^{+0.093}_{-0.19}}}
\newcommand{\fehausvalone}{\ensuremath{0.0195^{+0.0019}_{-0.0016}}}
\newcommand{\fehausvaltwo}{\ensuremath{0.0195^{+0.0019}_{-0.0016}}}
\newcommand{\fehausvalthree}{\ensuremath{0.0195^{+0.0019}_{-0.0016}}}
\newcommand{\fehausvalfour}{\ensuremath{0.0195^{+0.0019}_{-0.0016}}}
\newcommand{\fehausvalfive}{\ensuremath{0.0195^{+0.0019}_{-0.0016}}}
\newcommand{\fehausvalsix}{\ensuremath{0.0195^{+0.0019}_{-0.0016}}}
\newcommand{\tsonefourvalone}{\ensuremath{0.179^{+0.020}_{-0.010}}}
\newcommand{\tsonefourvaltwo}{\ensuremath{0.179^{+0.020}_{-0.010}}}
\newcommand{\tsonefourvalthree}{\ensuremath{0.179^{+0.020}_{-0.010}}}
\newcommand{\tsonefourvalfour}{\ensuremath{0.179^{+0.020}_{-0.010}}}
\newcommand{\tsonefourvalfive}{\ensuremath{0.179^{+0.020}_{-0.010}}}
\newcommand{\tsonefourvalsix}{\ensuremath{0.179^{+0.020}_{-0.010}}}
\newcommand{\tsfwhmvalone}{\ensuremath{0.159^{+0.020}_{-0.010}}}
\newcommand{\tsfwhmvaltwo}{\ensuremath{0.159^{+0.020}_{-0.010}}}
\newcommand{\tsfwhmvalthree}{\ensuremath{0.159^{+0.020}_{-0.010}}}
\newcommand{\tsfwhmvalfour}{\ensuremath{0.159^{+0.020}_{-0.010}}}
\newcommand{\tsfwhmvalfive}{\ensuremath{0.159^{+0.020}_{-0.010}}}
\newcommand{\tsfwhmvalsix}{\ensuremath{0.159^{+0.020}_{-0.010}}}
\newcommand{\dfehlfehasthreesixfehufehvalone}{\ensuremath{127.9^{+10.}_{-9.0}}}
\newcommand{\dfehlfehasthreesixfehufehvaltwo}{\ensuremath{127.9^{+10.}_{-9.0}}}
\newcommand{\dfehlfehasthreesixfehufehvalthree}{\ensuremath{127.9^{+10.}_{-9.0}}}
\newcommand{\dfehlfehasthreesixfehufehvalfour}{\ensuremath{127.9^{+10.}_{-9.0}}}
\newcommand{\dfehlfehasthreesixfehufehvalfive}{\ensuremath{127.9^{+10.}_{-9.0}}}
\newcommand{\dfehlfehasthreesixfehufehvalsix}{\ensuremath{127.9^{+10.}_{-9.0}}}
\newcommand{\dfehlfehasfourfivefehufehvalone}{\ensuremath{240^{+17}_{-15}}}
\newcommand{\dfehlfehasfourfivefehufehvaltwo}{\ensuremath{240^{+17}_{-15}}}
\newcommand{\dfehlfehasfourfivefehufehvalthree}{\ensuremath{240^{+17}_{-15}}}
\newcommand{\dfehlfehasfourfivefehufehvalfour}{\ensuremath{240^{+17}_{-15}}}
\newcommand{\dfehlfehasfourfivefehufehvalfive}{\ensuremath{240^{+17}_{-15}}}
\newcommand{\dfehlfehasfourfivefehufehvalsix}{\ensuremath{240^{+17}_{-15}}}
\newcommand{\fehopvalone}{\ensuremath{1.02^{+0.14}_{-0.13}}}
\newcommand{\fehopvaltwo}{\ensuremath{1.02^{+0.14}_{-0.13}}}
\newcommand{\fehopvalthree}{\ensuremath{1.02^{+0.14}_{-0.13}}}
\newcommand{\fehopvalfour}{\ensuremath{1.02^{+0.14}_{-0.13}}}
\newcommand{\fehopvalfive}{\ensuremath{1.02^{+0.14}_{-0.13}}}
\newcommand{\fehopvalsix}{\ensuremath{1.02^{+0.14}_{-0.13}}}
\newcommand{\loggpvalone}{\ensuremath{3.314^{+0.042}_{-0.045}}}
\newcommand{\loggpvaltwo}{\ensuremath{3.314^{+0.042}_{-0.045}}}
\newcommand{\loggpvalthree}{\ensuremath{3.314^{+0.042}_{-0.045}}}
\newcommand{\loggpvalfour}{\ensuremath{3.314^{+0.042}_{-0.045}}}
\newcommand{\loggpvalfive}{\ensuremath{3.314^{+0.042}_{-0.045}}}
\newcommand{\loggpvalsix}{\ensuremath{3.314^{+0.042}_{-0.045}}}
\newcommand{\tfehavalone}{\ensuremath{0.1568^{+0.0094}_{-0.0095}}}
\newcommand{\tfehavaltwo}{\ensuremath{0.1568^{+0.0094}_{-0.0095}}}
\newcommand{\tfehavalthree}{\ensuremath{0.1568^{+0.0094}_{-0.0095}}}
\newcommand{\tfehavalfour}{\ensuremath{0.1568^{+0.0094}_{-0.0095}}}
\newcommand{\tfehavalfive}{\ensuremath{0.1568^{+0.0094}_{-0.0095}}}
\newcommand{\tfehavalsix}{\ensuremath{0.1568^{+0.0094}_{-0.0095}}}
\newcommand{\fehavvalone}{\ensuremath{0.1552^{+0.0078}_{-0.0074}}}
\newcommand{\fehavvaltwo}{\ensuremath{0.1552^{+0.0078}_{-0.0074}}}
\newcommand{\fehavvalthree}{\ensuremath{0.1552^{+0.0078}_{-0.0074}}}
\newcommand{\fehavvalfour}{\ensuremath{0.1552^{+0.0078}_{-0.0074}}}
\newcommand{\fehavvalfive}{\ensuremath{0.1552^{+0.0078}_{-0.0074}}}
\newcommand{\fehavvalsix}{\ensuremath{0.1552^{+0.0078}_{-0.0074}}}
\newcommand{\tpvalone}{\ensuremath{2458495.8^{+1.2}_{-1.3}}}
\newcommand{\tpvaltwo}{\ensuremath{2458495.8^{+1.2}_{-1.3}}}
\newcommand{\tpvalthree}{\ensuremath{2458495.8^{+1.2}_{-1.3}}}
\newcommand{\tpvalfour}{\ensuremath{2458495.8^{+1.2}_{-1.3}}}
\newcommand{\tpvalfive}{\ensuremath{2458495.8^{+1.2}_{-1.3}}}
\newcommand{\tpvalsix}{\ensuremath{2458495.8^{+1.2}_{-1.3}}}
\newcommand{\tsvalone}{\ensuremath{2458501.03^{+0.14}_{-0.11}}}
\newcommand{\tsvaltwo}{\ensuremath{2458501.03^{+0.14}_{-0.11}}}
\newcommand{\tsvalthree}{\ensuremath{2458501.03^{+0.14}_{-0.11}}}
\newcommand{\tsvalfour}{\ensuremath{2458501.03^{+0.14}_{-0.11}}}
\newcommand{\tsvalfive}{\ensuremath{2458501.03^{+0.14}_{-0.11}}}
\newcommand{\tsvalsix}{\ensuremath{2458501.03^{+0.14}_{-0.11}}}
\newcommand{\tavalone}{\ensuremath{2458493.51^{+0.21}_{-0.14}}}
\newcommand{\tavaltwo}{\ensuremath{2458493.51^{+0.21}_{-0.14}}}
\newcommand{\tavalthree}{\ensuremath{2458493.51^{+0.21}_{-0.14}}}
\newcommand{\tavalfour}{\ensuremath{2458493.51^{+0.21}_{-0.14}}}
\newcommand{\tavalfive}{\ensuremath{2458493.51^{+0.21}_{-0.14}}}
\newcommand{\tavalsix}{\ensuremath{2458493.51^{+0.21}_{-0.14}}}
\newcommand{\tdvalone}{\ensuremath{2458498.36^{+0.12}_{-0.20}}}
\newcommand{\tdvaltwo}{\ensuremath{2458498.36^{+0.12}_{-0.20}}}
\newcommand{\tdvalthree}{\ensuremath{2458498.36^{+0.12}_{-0.20}}}
\newcommand{\tdvalfour}{\ensuremath{2458498.36^{+0.12}_{-0.20}}}
\newcommand{\tdvalfive}{\ensuremath{2458498.36^{+0.12}_{-0.20}}}
\newcommand{\tdvalsix}{\ensuremath{2458498.36^{+0.12}_{-0.20}}}
\newcommand{\vcvvalone}{\ensuremath{0.963^{+0.039}_{-0.055}}}
\newcommand{\vcvvaltwo}{\ensuremath{0.963^{+0.039}_{-0.055}}}
\newcommand{\vcvvalthree}{\ensuremath{0.963^{+0.039}_{-0.055}}}
\newcommand{\vcvvalfour}{\ensuremath{0.963^{+0.039}_{-0.055}}}
\newcommand{\vcvvalfive}{\ensuremath{0.963^{+0.039}_{-0.055}}}
\newcommand{\vcvvalsix}{\ensuremath{0.963^{+0.039}_{-0.055}}}
\newcommand{\cosofehgastarvalone}{\ensuremath{0.002^{+0.022}_{-0.018}}}
\newcommand{\cosofehgastarvaltwo}{\ensuremath{0.002^{+0.022}_{-0.018}}}
\newcommand{\cosofehgastarvalthree}{\ensuremath{0.002^{+0.022}_{-0.018}}}
\newcommand{\cosofehgastarvalfour}{\ensuremath{0.002^{+0.022}_{-0.018}}}
\newcommand{\cosofehgastarvalfive}{\ensuremath{0.002^{+0.022}_{-0.018}}}
\newcommand{\cosofehgastarvalsix}{\ensuremath{0.002^{+0.022}_{-0.018}}}
\newcommand{\sinofehgastarvalone}{\ensuremath{0.038^{+0.059}_{-0.039}}}
\newcommand{\sinofehgastarvaltwo}{\ensuremath{0.038^{+0.059}_{-0.039}}}
\newcommand{\sinofehgastarvalthree}{\ensuremath{0.038^{+0.059}_{-0.039}}}
\newcommand{\sinofehgastarvalfour}{\ensuremath{0.038^{+0.059}_{-0.039}}}
\newcommand{\sinofehgastarvalfive}{\ensuremath{0.038^{+0.059}_{-0.039}}}
\newcommand{\sinofehgastarvalsix}{\ensuremath{0.038^{+0.059}_{-0.039}}}
\newcommand{\mpsinfehivalone}{\ensuremath{0.847^{+0.052}_{-0.049}}}
\newcommand{\mpsinfehivaltwo}{\ensuremath{0.847^{+0.052}_{-0.049}}}
\newcommand{\mpsinfehivalthree}{\ensuremath{0.847^{+0.052}_{-0.049}}}
\newcommand{\mpsinfehivalfour}{\ensuremath{0.847^{+0.052}_{-0.049}}}
\newcommand{\mpsinfehivalfive}{\ensuremath{0.847^{+0.052}_{-0.049}}}
\newcommand{\mpsinfehivalsix}{\ensuremath{0.847^{+0.052}_{-0.049}}}
\newcommand{\mpmvalone}{\ensuremath{0.000830^{+0.000042}_{-0.000044}}}
\newcommand{\mpmvaltwo}{\ensuremath{0.000830^{+0.000042}_{-0.000044}}}
\newcommand{\mpmvalthree}{\ensuremath{0.000830^{+0.000042}_{-0.000044}}}
\newcommand{\mpmvalfour}{\ensuremath{0.000830^{+0.000042}_{-0.000044}}}
\newcommand{\mpmvalfive}{\ensuremath{0.000830^{+0.000042}_{-0.000044}}}
\newcommand{\mpmvalsix}{\ensuremath{0.000830^{+0.000042}_{-0.000044}}}
\newcommand{\drvalone}{\ensuremath{18.4^{+1.2}_{-1.4}}}
\newcommand{\drvaltwo}{\ensuremath{18.4^{+1.2}_{-1.4}}}
\newcommand{\drvalthree}{\ensuremath{18.4^{+1.2}_{-1.4}}}
\newcommand{\drvalfour}{\ensuremath{18.4^{+1.2}_{-1.4}}}
\newcommand{\drvalfive}{\ensuremath{18.4^{+1.2}_{-1.4}}}
\newcommand{\drvalsix}{\ensuremath{18.4^{+1.2}_{-1.4}}}
\newcommand{\ptvalone}{\ensuremath{0.0487^{+0.0041}_{-0.0029}}}
\newcommand{\ptvaltwo}{\ensuremath{0.0487^{+0.0041}_{-0.0029}}}
\newcommand{\ptvalthree}{\ensuremath{0.0487^{+0.0041}_{-0.0029}}}
\newcommand{\ptvalfour}{\ensuremath{0.0487^{+0.0041}_{-0.0029}}}
\newcommand{\ptvalfive}{\ensuremath{0.0487^{+0.0041}_{-0.0029}}}
\newcommand{\ptvalsix}{\ensuremath{0.0487^{+0.0041}_{-0.0029}}}
\newcommand{\ptgvalone}{\ensuremath{0.0597^{+0.0049}_{-0.0036}}}
\newcommand{\ptgvaltwo}{\ensuremath{0.0597^{+0.0049}_{-0.0036}}}
\newcommand{\ptgvalthree}{\ensuremath{0.0597^{+0.0049}_{-0.0036}}}
\newcommand{\ptgvalfour}{\ensuremath{0.0597^{+0.0049}_{-0.0036}}}
\newcommand{\ptgvalfive}{\ensuremath{0.0597^{+0.0049}_{-0.0036}}}
\newcommand{\ptgvalsix}{\ensuremath{0.0597^{+0.0049}_{-0.0036}}}
\newcommand{\psvalone}{\ensuremath{0.0448^{+0.0025}_{-0.0022}}}
\newcommand{\psvaltwo}{\ensuremath{0.0448^{+0.0025}_{-0.0022}}}
\newcommand{\psvalthree}{\ensuremath{0.0448^{+0.0025}_{-0.0022}}}
\newcommand{\psvalfour}{\ensuremath{0.0448^{+0.0025}_{-0.0022}}}
\newcommand{\psvalfive}{\ensuremath{0.0448^{+0.0025}_{-0.0022}}}
\newcommand{\psvalsix}{\ensuremath{0.0448^{+0.0025}_{-0.0022}}}
\newcommand{\psgvalone}{\ensuremath{0.0549^{+0.0033}_{-0.0029}}}
\newcommand{\psgvaltwo}{\ensuremath{0.0549^{+0.0033}_{-0.0029}}}
\newcommand{\psgvalthree}{\ensuremath{0.0549^{+0.0033}_{-0.0029}}}
\newcommand{\psgvalfour}{\ensuremath{0.0549^{+0.0033}_{-0.0029}}}
\newcommand{\psgvalfive}{\ensuremath{0.0549^{+0.0033}_{-0.0029}}}
\newcommand{\psgvalsix}{\ensuremath{0.0549^{+0.0033}_{-0.0029}}}
\newcommand{\uonevalone}{\ensuremath{0.391\pm0.047}}
\newcommand{\uonevaltwo}{\ensuremath{0.391\pm0.047}}
\newcommand{\uonevalthree}{\ensuremath{0.391\pm0.047}}
\newcommand{\uonevalfour}{\ensuremath{0.391\pm0.047}}
\newcommand{\uonevalfive}{\ensuremath{0.391\pm0.047}}
\newcommand{\uonevalsix}{\ensuremath{0.391\pm0.047}}
\newcommand{\utwovalone}{\ensuremath{0.252^{+0.049}_{-0.048}}}
\newcommand{\utwovaltwo}{\ensuremath{0.252^{+0.049}_{-0.048}}}
\newcommand{\utwovalthree}{\ensuremath{0.252^{+0.049}_{-0.048}}}
\newcommand{\utwovalfour}{\ensuremath{0.252^{+0.049}_{-0.048}}}
\newcommand{\utwovalfive}{\ensuremath{0.252^{+0.049}_{-0.048}}}
\newcommand{\utwovalsix}{\ensuremath{0.252^{+0.049}_{-0.048}}}
\newcommand{\advalone}{\ensuremath{--}}
\newcommand{\advaltwo}{\ensuremath{--}}
\newcommand{\advalthree}{\ensuremath{--}}
\newcommand{\advalfour}{\ensuremath{--}}
\newcommand{\advalfive}{\ensuremath{--}}
\newcommand{\advalsix}{\ensuremath{--}}
\newcommand{\gafehafehlvalone}{\ensuremath{19385.4\pm6.9}}
\newcommand{\gafehafehlvaltwo}{\ensuremath{19385.4\pm6.9}}
\newcommand{\gafehafehlvalthree}{\ensuremath{19385.4\pm6.9}}
\newcommand{\gafehafehlvalfour}{\ensuremath{19385.4\pm6.9}}
\newcommand{\gafehafehlvalfive}{\ensuremath{19385.4\pm6.9}}
\newcommand{\gafehafehlvalsix}{\ensuremath{19385.4\pm6.9}}
\newcommand{\sigfehajvalone}{\ensuremath{31.7^{+6.4}_{-5.4}}}
\newcommand{\sigfehajvaltwo}{\ensuremath{31.7^{+6.4}_{-5.4}}}
\newcommand{\sigfehajvalthree}{\ensuremath{31.7^{+6.4}_{-5.4}}}
\newcommand{\sigfehajvalfour}{\ensuremath{31.7^{+6.4}_{-5.4}}}
\newcommand{\sigfehajvalfive}{\ensuremath{31.7^{+6.4}_{-5.4}}}
\newcommand{\sigfehajvalsix}{\ensuremath{31.7^{+6.4}_{-5.4}}}
\newcommand{\sigfehajtwovalone}{\ensuremath{1000^{+440}_{-310}}}
\newcommand{\sigfehajtwovaltwo}{\ensuremath{1000^{+440}_{-310}}}
\newcommand{\sigfehajtwovalthree}{\ensuremath{1000^{+440}_{-310}}}
\newcommand{\sigfehajtwovalfour}{\ensuremath{1000^{+440}_{-310}}}
\newcommand{\sigfehajtwovalfive}{\ensuremath{1000^{+440}_{-310}}}
\newcommand{\sigfehajtwovalsix}{\ensuremath{1000^{+440}_{-310}}}
\newcommand{\sigfehatwovalone}{\ensuremath{-0.000000006^{+0.000000024}_{-0.000000019}}}
\newcommand{\sigfehatwovaltwo}{\ensuremath{-0.000000006^{+0.000000024}_{-0.000000019}}}
\newcommand{\sigfehatwovalthree}{\ensuremath{-0.000000006^{+0.000000024}_{-0.000000019}}}
\newcommand{\sigfehatwovalfour}{\ensuremath{-0.000000006^{+0.000000024}_{-0.000000019}}}
\newcommand{\sigfehatwovalfive}{\ensuremath{-0.000000006^{+0.000000024}_{-0.000000019}}}
\newcommand{\sigfehatwovalsix}{\ensuremath{-0.000000006^{+0.000000024}_{-0.000000019}}}
\newcommand{\fzerovalone}{\ensuremath{1.000012\pm0.000045}}
\newcommand{\fzerovaltwo}{\ensuremath{1.000012\pm0.000045}}
\newcommand{\fzerovalthree}{\ensuremath{1.000012\pm0.000045}}
\newcommand{\fzerovalfour}{\ensuremath{1.000012\pm0.000045}}
\newcommand{\fzerovalfive}{\ensuremath{1.000012\pm0.000045}}
\newcommand{\fzerovalsix}{\ensuremath{1.000012\pm0.000045}}
